Enhanced Absorption in thin and ultrathin silicon films by 3D photonic band gap back reflectors

Since thin-film silicon solar cells have limited optical absorption, we explore the effect of a nanostructured back reflector to recycle the unabsorbed light. As a back reflector we investigate a 3D photonic band gap crystal made from silicon that is readily integrated with the thin films. We numerically obtain the optical properties by solving the 3D time-harmonic Maxwell equations using the finite-element method, and model silicon with experimentally determined optical constants. The absorption enhancement relevant for photovoltaics is obtained by weighting the absorption spectra with the AM 1.5 standard solar spectrum. We study thin films either thicker ($L_{Si} = 2400$ nm) or much thinner ($L_{Si} = 80$ nm) than the wavelength of light. At $L_{Si} = 2400$ nm, the 3D photonic band gap crystal enhances the spectrally averaged ($\lambda = 680$ nm to $880$ nm) silicon absorption by $2.22$x (s-pol.) to $2.45$x (p-pol.), which exceeds the enhancement of a perfect metal back reflector ($1.47$ to $1.56$x). The absorption is enhanced by the (i) broadband angle and polarization-independent reflectivity in the 3D photonic band gap, and (ii) the excitation of many guided modes in the film by the crystal's surface diffraction leading to enhanced path lengths. At $L_{Si} = 80$ nm, the photonic crystal back reflector yields a striking average absorption enhancement of $9.15$x, much more than $0.83$x for a perfect metal, which is due to a remarkable guided mode confined within the combined thickness of the thin film and the photonic crystal's Bragg attenuation length. The broad bandwidth of the 3D photonic band gap leads to the back reflector's Bragg attenuation length being much shorter than the silicon absorption length. Consequently, light is confined inside the thin film and the absorption enhancements are not due to the additional thickness of the photonic crystal back reflector.

==> 1_Resubmission1/Report_referee1_referee2.tex <==

Reviewer 1:

The manuscript reports on calculations of absorption in thin silicon films with backreflectors made of 3D inverse woodpile photonic crystals with a complete photonic band gap. Strong absorption enhancement due to the 3D photonic band structure is demonstrated, thanks to full reflection and (for the thicker film, 2400 nm) to the excitation of guided modes. The physics behind the calculated results is explained in detail. The manuscript contains new results in the field of photonics for photovoltaics that may be worth publishing, however, there is a large body of literature in the field and the authors should better demonstrate the interest of their results for the community. I think the manuscript should be revised along the following comments:

1. The authors always mention “absorption enhancement”, but they almost never quote the absolute absorption, and they never mention the quantity that is most relevant for PV cells, namely the short-circuit current.

2. How can the use of silicon backreflector be compatible with carrier collection at the rear interface?

3. The authors should compare their results with the known light-trapping limits, e.g. their Fig. 12 with Fig. 1 of Adv. Phys. X 4, 1548305 (2018) https://doi.org/10.1080/23746149.2018.1548305

4. There is a series of papers on 3D photonic crystals as reflectors for thin-films silicon solar cells, see e.g. J. of Optics 14, 024003 (2012) https://doi.org/10.1088/2040-8978/14/2/024003; Optics Express 21, A528-A538 (2013) https://doi.org/10.1364/OE.21.00A528


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


Scope of the journal :
This manuscript reports the study of 3D photonic band gap back reflectors to enhance light absorption in thin silicon films with a targeted application to ultrathin silicon solar cells. It thereby fits well within the scope of Energy and Environmental Optics Express.

Novelty/impact :
Enhancing light absorption in thin films is a key issue for next generation photovoltaics as ultrathin solar cells are an envisioned path to reduce material usage and enable low weight or flexible applications. In this context, the concept proposed by the authors of replacing metal back reflectors by 3D photonic band gap crystal reflectors is quite original. Their photonic band gap solution offers potential advantages over the metallic counterpart such as a better reflectivity on a broad spectral band, an additional light-trapping effect due to the generation of guided modes and a technological integration facilitated by the all-silicon approach.
        In my opinion, the main weakness of the manuscript is the gap remaining between the concept proposed and studied by the authors and its practical application to a real solar cell. In order to insist on the feasibility of a silicon solar cell integrating a 3D photonic band gap reflector, here are some suggestions to enrich  the section « Practical considerations for devices » :
(1) A schematic of the complete cell architecture the authors envision could be added, including in particular the metallic back contact. Indeed, though the concept proposed enables an all-silicon approach, a back electrical contact is needed and should be integrated on the 3D photonic band gap reflector.
(2) The impact of adding doped layers for carrier collection should also be discussed.
(3) Furthermore, in the current version of the manuscript, several thicknesses of the silicon film are studied, in particular a thick cell (2400 nm) and an ultrathin cell (80 nm), in this order. Though both are interesting from an optical point of view to understand the physics involved, 80 nm-thick silicon solar cells do not seem very likely to be realized experimentally. The authors should highlight the cell architecture most likely to lead to a practical realization. Likewise, it could be better to modify the outline of the manuscript to end on the thick cell.

Technical content :
The study reported in the article is quite interesting and the conclusions on the impact of the 3D photonic band gap reflector on light absorption in thin film silicon solar cells are well supported by the data presented. The work presented is also well put in context in the introduction. However, I find that the manuscript is missing a comparison of the results presented with state-of-the-art works on similar concepts to properly highlight their significance for the research field. The authors use as a main figure of merit the absorption enhancement compared to a reference with no back reflector. Though this is interesting from an optical point of view, it does not allow a proper comparison with existing literature on thin film silicon solar cells integrating nanophotonic strategies such as Ref. 30. It would be interesting to assess the theoretical short-circuit current density of a cell integrating the proposed 3D photonic band gap reflector (as done in Massiot et al. Nature Energy 5, 959-972 (2020) for instance). In addition to allowing for a proper comparison with similar works, it would also be another element to show the potential of the concept for silicon solar cells and thus increase the impact of the article.

Quality of presentation :
The manuscript is well written and quite understandable. Nevertheless, here are some suggestions to improve the article :
(1) Including a 3D schematic of the inverted woodpile structure would help the reader to get a better picture of the studied structure.
(2) Likewise, schematics of the structures studied could be inserted in the figures with the calculated spectra.
(3) l.39 : the expression « economical step » is not clear.
(4) l.64 : the authors use « recently » to refer to some works among which one work from 1984 (Ref.22).


==> 1_Resubmission1/_to_referee_1.tex <==
Optics Express Manuscript 435412 by Devashish Sharma, Shakeeb Bin Hasan, Rebecca Saive, Jaap J. W. van der Vegt, and Willem L. Vos
===================================
Response to the report of Referee 1
===================================

GENERAL COMMENT-0: 
The manuscript reports on calculations of absorption in thin silicon films with backreflectors made of 3D inverse woodpile photonic crystals with a complete photonic band gap. Strong absorption enhancement due to the 3D photonic band structure is demonstrated, thanks to full reflection and (for the thicker film, 2400 nm) to the excitation of guided modes. The physics behind the calculated results is explained in detail. The manuscript contains new results in the field of photonics for photovoltaics that may be worth publishing, however, there is a large body of literature in the field and the authors should better demonstrate the interest of their results for the community. I think the manuscript should be revised along the following comments:

REPLY-0:
We are pleased with the positive comments of the Referee. We appreciate the constructive and helpful comments to improve our manuscript. Therefore, we resubmit a revised version of our manuscript. Below we address the detailed comments. 

COMMENT-1: The authors always mention “absorption enhancement”, but they almost never quote the absolute absorption, and they never mention the quantity that is most relevant for PV cells, namely the short-circuit current.

REPLY-1: A) To clarify for the readers, we emphasize more strongly that Figs. 5 and 8 show the absolute absorption in percentage. 
B) Regarding the short-circuit current $J_{SC}$, we thank the Referee for his suggestion. We now describe the short-circuit current $J_{SC}$ in Appendix D, and our results in terms of the short-circuit current are given in Tables 1 and 2. This comparison shows that our back reflector exceeds bare Si results by a factor 3x. 

COMMENT-2: How can the use of silicon backreflector be compatible with carrier collection at the rear interface?

REPLY-2: We thank the Referee for this interesting and practical suggestion. The scope of our paper is to study an optical effect, namely how to enhance the optical absorption of thin Si layers, with a sharp eye on applications in solar cells. To meet the Referee's question we sketch a simple possible back contact in Fig. 1. 

COMMENT-3. The authors should compare their results with the known light-trapping limits, e.g. their Fig. 12 with Fig. 1 of Adv. Phys. X 4, 1548305 (2018) https://doi.org/10.1080/23746149.2018.1548305

REPLY-3: We thank the Referee for suggesting the comparison of our results with other light-trapping limits. Therefore, we have plotted the absorption according to the Lambertian scattering model in Figs. 5 and 8. We thank the Referee for pointing out the Andreani et al. paper (which is added as a reference 18.) In contrast to Andreani et al, the scope of our paper is to enhance absorption in the range (>700 nm) where Si absorbs very weakly, we do not study the whole solar range (in contrast to Andreani et al.) Therefore, it is not meaningful to directly compare our results to theirs. 

COMMENT-4. There is a series of papers on 3D photonic crystals as reflectors for thin-films silicon solar cells, see e.g. J. of Optics 14, 024003 (2012) https://doi.org/10.1088/2040-8978/14/2/024003; Optics Express 21, A528-A538 (2013) https://doi.org/10.1364/OE.21.00A528

REPLY-4: We thank the Referee for pointing out these interesting papers (and we apologize for our oversight). We have added these papers as references 40 and 41. 


==> 1_Resubmission1/_to_referee_2.tex <==
Optics Express Manuscript 435412 by Devashish Sharma, Shakeeb Bin Hasan, Rebecca Saive, Jaap J. W. van der Vegt, and Willem L. Vos
===================================
Response to the report of Referee 2
===================================


GENERAL COMMENT-0:
Scope of the journal :
This manuscript reports the study of 3D photonic band gap back reflectors to enhance light absorption in thin silicon films with a targeted application to ultrathin silicon solar cells. It thereby fits well within the scope of Energy and Environmental Optics Express.

Novelty/impact :
Enhancing light absorption in thin films is a key issue for next generation photovoltaics as ultrathin solar cells are an envisioned path to reduce material usage and enable low weight or flexible applications. In this context, the concept proposed by the authors of replacing metal back reflectors by 3D photonic band gap crystal reflectors is quite original. Their photonic band gap solution offers potential advantages over the metallic counterpart such as a better reflectivity on a broad spectral band, an additional light-trapping effect due to the generation of guided modes and a technological integration facilitated by the all-silicon approach.
In my opinion, the main weakness of the manuscript is the gap remaining between the concept proposed and studied by the authors and its practical application to a real solar cell. In order to insist on the feasibility of a silicon solar cell integrating a 3D photonic band gap reflector, here are some suggestions to enrich  the section « Practical considerations for devices » :

REPLY-0:
We thank the Referee for the positive evaluation. We appreciate the constructive and useful comments to improve our manuscript. Therefore, we hereby resubmit a revised version of our manuscript. We now address the detailed remarks. 

COMMENT-1: A schematic of the complete cell architecture the authors envision could be added, including in particular the metallic back contact. Indeed, though the concept proposed enables an all-silicon approach, a back electrical contact is needed and should be integrated on the 3D photonic band gap reflector.

REPLY-1: We thank the Referee for the interesting suggestion. The scope of our paper is to study an optical effect, namely to enhance the absorption of thin Si layers, with a keen eye on applications in solar cells. To accommodate the Referee's question, we sketch possible back contacts into the generic design in Fig. 1. Moreover, to emphasize the new optical results, we have at a few instances replaced our over-enthusiastic use of "solar cell" by "thin silicon film". 
In practice, integrating such components to Si devices is well feasible, as discussed in section 4.3. 

COMMENT-2: The impact of adding doped layers for carrier collection should also be discussed. 

REPLY-2: If one considers a doping level of 10^16 cm^-3, this already gives substantial mobility. Fortunately, from the famous semiconductor data collection of the Ioffe Institute ("SVM") we learn that this doping level gives a very small change in optical properties (Real(nSi), Im(nSi)), as is explained in Appendix C. 

COMMENT-3: Furthermore, in the current version of the manuscript, several thicknesses of the silicon film are studied, in particular a thick cell (2400 nm) and an ultrathin cell (80 nm), in this order. Though both are interesting from an optical point of view to understand the physics involved, 80 nm-thick silicon solar cells do not seem very likely to be realized experimentally. The authors should highlight the cell architecture most likely to lead to a practical realization. Likewise, it could be better to modify the outline of the manuscript to end on the thick cell. 

REPLY-3: A) Regarding the choice of different thin films, we  recently had the pleasure to attend the online OSA Symposium "40 years of light management in solar cells", part of the 2021 OSA Advanced Photonics Congress. Here legendary scientist prof. Eli Yablonovitch discussed similar thin Si solar cells in his keynote address (https://www.osa.org/en-us/meetings/osa_meetings/advanced_photonics_congress/program/symposia/). In view of this famous scientist's talk, we feel that our study of the ultrathin 80 nm film are warranted. 
Moreover, the Massiot et al review paper (Ref. 68) also emphasizes research in the direction of ultrathin silicon solar cells. Remarkably, in this case case, the 3D photonic back reflector outperforms the Lambertian limit at several resonances (even without front surface optimization). And this is what motivated us to present ultrathin results. 
B) To address the Referee's comment about practical realization, we have added material on solar cell specifics, e.g., edited the Intro (4th sentence), updated Fig. 1 and Appendices C and D. 

COMMENT-4 
Technical content :
The study reported in the article is quite interesting and the conclusions on the impact of the 3D photonic band gap reflector on light absorption in thin film silicon solar cells are well supported by the data presented. The work presented is also well put in context in the introduction. However, I find that the manuscript is missing a comparison of the results presented with state-of-the-art works on similar concepts to properly highlight their significance for the research field. The authors use as a main figure of merit the absorption enhancement compared to a reference with no back reflector. Though this is interesting from an optical point of view, it does not allow a proper comparison with existing literature on thin film silicon solar cells integrating nanophotonic strategies such as Ref. 30. It would be interesting to assess the theoretical short-circuit current density of a cell integrating the proposed 3D photonic band gap reflector (as done in Massiot et al. Nature Energy 5, 959-972 (2020) for instance). In addition to allowing for a proper comparison with similar works, it would also be another element to show the potential of the concept for silicon solar cells and thus increase the impact of the article.

REPLY-4: We thank the Referee for the positive assessment, and for reminding us of the Massiot et al paper, we are sorry that we had missed it; it is now inserted as new Reference 68. 
We have computed the short-circuit current (see Appendix D) and added a discussion about it. 

COMMENT-5: 
Quality of presentation :
The manuscript is well written and quite understandable. Nevertheless, here are some suggestions to improve the article :
(1) Including a 3D schematic of the inverted woodpile structure would  appreciate crystal structure, so I keep voting for my suggestion below. 

REPLY-5: We appreciate the comment of the Referee to elucidate the 3D inverse woodpile photonic crystal structure and have added it in the new Fig. 2(a) (and matching description). 

COMMENT-6: (2) Likewise, schematics of the structures studied could be inserted in the figures with the calculated spectra. 

REPLY-6: The Referee's comment made us realize our unclarity in several figures, especially Fig.3 where "thin film" was undefined. To clarify the figures, we improved the legends to list the film thickness. 

COMMENT-7: (3) l.39 : the expression « economical step » is not clear.

REPLY-7: We agree that the statement was unclear. We have rewritten the very 1st sentence of the manuscript, thereby taking into account the latest developments with the IPCC report on the ongoing climate crisis. 

COMMENT-8: (4) l.64 : the authors use « recently » to refer to some works among which one work from 1984 (Ref.22).

REPLY-8: We thank the referee for pointing out the linguistic error. We replaced the word "recently" with "notably".


